SRIF: Semantic Shape Registration Empowered by Diffusion-based Image Morphing and Flow Estimation

In this paper, we propose SRIF, a novel Semantic shape Registration framework based on diffusion-based Image morphing and Flow estimation. More concretely, given a pair of extrinsically aligned shapes, we first render them from multi-views, and then utilize an image interpolation framework based on diffusion models to generate sequences of intermediate images between them. The images are later fed into a dynamic 3D Gaussian splatting framework, with which we reconstruct and post-process for intermediate point clouds respecting the image morphing processing. In the end, tailored for the above, we propose a novel registration module to estimate continuous normalizing flow, which deforms source shape consistently towards the target, with intermediate point clouds as weak guidance. Our key insight is to leverage large vision models (LVMs) to associate shapes and therefore obtain much richer semantic information on the relationship between shapes than the ad-hoc feature extraction and alignment. As a consequence, SRIF achieves high-quality dense correspondences on challenging shape pairs, but also delivers smooth, semantically meaningful interpolation in between. Empirical evidence justifies the effectiveness and superiority of our method as well as specific design choices. The code is released at https://github.com/rqhuang88/SRIF.

==> Figs-new/teaser.tex <==
\begin{figure*}[h!]
  \begin{center}
\includegraphics[width=17.5cm]{Figs-new/teaser3.png}
  \end{center}
\caption{ }
\label{fig:teaser}
\end{figure*}

==> Figs/ablation.tex <==
\begin{figure}[t!]
  \begin{center}
\includegraphics[width=8.5cm]{Figs/ablation_2.png}
  \end{center}
\caption{We show the ablation results performed on a pair from \texttt{Fourleg} shape collection. }
\label{fig:ablation}
\end{figure}

==> Figs/application.tex <==
\begin{figure}[t!]
  \begin{center}
\includegraphics[width=8.5cm]{Figs/application.png}
  \end{center}
\caption{Our sequential registration allows for driving the intermediate meshes with poses performed by the source shape. }
\label{fig:application}
\end{figure}

==> Figs/fourleg.tex <==
\begin{figure}[t!]
  \begin{center}
\includegraphics[width=8.5cm]{Figs/fourleg.png}
  \end{center}
\caption{Part of registration results on \texttt{Fourleg} shape collection. While being landmark-annotation-free, our method delivers comparable result with respect to SMAT~\cite{EG}, the state-of-the-art compatible remeshing technique.  }
\label{fig:fourleg}
\end{figure}

==> Figs/insight.tex <==
\begin{figure}[t!]
  \begin{center}
\includegraphics[width=8.5cm]{Figs/Insight.png}
  \end{center}
\caption{The straightforward output of Deformable 3D-GS contains large amount of inner points (left-most), after our proposed post-processing, points that close to the underlying surface are extracted (middle-right). The meshes in the middle-right and left-most are registration results based on the down-sampled points from the original point cloud and the post-processed one. Note that we visualize half of the point clouds for better inspection. }
\label{fig:Insight}
\end{figure}

==> Figs/render.tex <==
\begin{figure}[t!]
  \begin{center}
\includegraphics[width=8.5cm]{Figs/render.png}
  \end{center}
\caption{We respectively render meshes and the corresponding vertex sets using Open3D render with the color scheme detailed in Sec.~\ref{sec:render}. The number attached to the top-right of each image on the bottom row indicates the PSNR score regarding its counterpart on the top row. From left to right, the number of vertices are $46k, 25k, \mbox{and} 7k$. }
\label{fig:render}
\end{figure}

==> Figs/teaser.tex <==
\begin{figure}[t!]
  \begin{center}
\includegraphics[width=8.5cm]{Figs/teasersig.png}
  \end{center}
\caption{We propose \textbf{HRIM}, an autonomous framework for heterogeneous 3D shape registration, which produces high-quality correspondences (right) without either user-defined constraints or category-specific 3D data pre-training (left). }
\label{fig:teaser}
\end{figure}

==> Tabs/fourleg.tex <==
\begin{table}[!t]
\caption{Comparison to baselines on Fourleg dataset. ↑ indicates higher is better and ↓ indicates lower is better.}\label{table:1}
\centering
\begin{tabular}
{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline

           & Dirichlet ↓ & Cov. ↑        & Chamfer ↓          & Lmks. Err. ↓       \\ \hline
NDP        & 936.6778          & 0.5724          & 0.0168          & 0.4495          \\
NeuroMorph & 23.4818           & 0.3988          & 0.0059          & 0.0912          \\
EBCM\tablefootnote{EBCM only converges in $3$ out of $19$ pairs within $15$-hour budget, therefore we ignore it in this table. }       &    -               &    -             &   -              &   -              \\
SMAT       & \textbf{5.6113}   & 0.5664          & 0.0071          & \textbf{0.0011} \\
Ours       & 6.7018            & \textbf{0.6647} & \textbf{0.0055} & 0.0737          \\ \hline
\end{tabular}
\end{table}

==> Tabs/time.tex <==
\begin{table}[!t]
\caption{\textcolor{blue}{We compare the running times with baselines, with all methods measured on the same device while optimizing the running time for the same pair of shapes.}}\label{table:time}
\centering
% \setlength{\tabcolsep}{4pt}
% \resizebox{\textwidth}{12mm}{
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
                   & Maptree & BIM & SS & NM & ENIGMA & Ours \\ \hline
Time (min) & 1       & 1   & 5           & 1          & 20     & 40   \\ \hline
\end{tabular}
% \vspace{1em}
\end{table}

==> figures.tex <==
% \input{Figs/zoo_1}
% \input{Figs/zoo_2}

% \input{Figs-new/interpolation}          
